Local Dampening: Differential Privacy for Non-numeric Queries via Local Sensitivity

Differential privacy is the state-of-the-art formal definition for data release under strong privacy guarantees. A variety of mechanisms have been proposed in the literature for releasing the output of numeric queries (e.g., the Laplace mechanism and smooth sensitivity mechanism). Those mechanisms guarantee differential privacy by adding noise to the true query's output. The amount of noise added is calibrated by the notions of global sensitivity and local sensitivity of the query that measure the impact of the addition or removal of an individual on the query's output. Mechanisms that use local sensitivity add less noise and, consequently, have a more accurate answer. However, although there has been some work on generic mechanisms for releasing the output of non-numeric queries using global sensitivity (e.g., the Exponential mechanism), the literature lacks generic mechanisms for releasing the output of non-numeric queries using local sensitivity to reduce the noise in the query's output. In this work, we remedy this shortcoming and present the local dampening mechanism. We adapt the notion of local sensitivity for the non-numeric setting and leverage it to design a generic non-numeric mechanism. We provide theoretical comparisons to the exponential mechanism and show under which conditions the local dampening mechanism is more accurate than the exponential mechanism. We illustrate the effectiveness of the local dampening mechanism by applying it to three diverse problems: (i) percentile selection problem. We report the p-th element in the database; (ii) Influential node analysis. Given an influence metric, we release the top-k most influential nodes while preserving the privacy of the relationship between nodes in the network; (iii) Decision tree induction. We provide a private adaptation to the ID3 algorithm to build decision trees from a given tabular dataset.

==> figures/dampening_function.tex <==
\begin{figure*}
	\centering
	\begin{tikzpicture}
		\foreach \x/\y [count=\xi from 1] in {0.7/0.8, 1.4/2.3, 2.1/5}{
			\draw [ultra thick] (-.1,\x) -- (.1,\x);
			\draw [ultra thick] (-.1,-\x) -- (.1,-\x);
			\node at (-.3,\x) {\xi};
			\node at (.3,-\x) {-\xi};
			\draw [fill] (\y,\x) circle [radius=0.08];
			\draw [fill] (-\y,-\x) circle [radius=0.08];
			\draw [dashed] (0,\x) -- (\y,\x);
			\draw [dashed] (0,-\x) -- (-\y,-\x);
			\draw [dashed] (\y, 0) -- (\y,\x);
			\draw [dashed] (-\y, 0) -- (-\y,-\x);
			% \pgfmathtruncatemacro{\xii}{\xi - 1}            
			% \node at (-\y, 0.3) { $-\sum_{i=0}^{\xii}\delta(i,r)$};
		}
		\node at (1.1, -0.3) { $\sum_{i=0}^{0}\delta(i,r)$};
		\node at (2.9, -0.3) { $\sum_{i=0}^{1}\delta(i,r)$};
		\node at (5.1, -0.3) { $\sum_{i=0}^{2}\delta(i,r)$};
		\node at (-1., 0.3) { $-\sum_{i=0}^{0}\delta(i,r)$};
		\node at (-3., 0.3) { $-\sum_{i=0}^{1}\delta(i,r)$};
		\node at (-5.3, 0.3) { $-\sum_{i=0}^{2}\delta(i,r)$};
		\draw [thick] (0,0) -- (0.8,0.7) -- (2.3, 1.4) -- (5, 2.1);
		\draw [thick] (0,0) -- (-0.8,-0.7) -- (-2.3, -1.4) -- (-5, -2.1);
		\draw [->, thick] (0,-2.3) -- (0,3);
		\draw [->, thick] (-6.4,0) -- (6.4,0);
		\node at (.3,2.8) {$D$};
		\node at (6,.3) {$u$};
	\end{tikzpicture}    
    \caption{Dampening function $D_{u, \delta^u}$}
    \label{fig:dampening}
\end{figure*}

==> sections/10_introduction2.tex <==
\section{Introduction}
\label{section:introduction}

Many corporations, organizations, and government offices have been gathering data over the last decades. The entity that manages this data is called \textit{curator}. The curator is a trusted tier that collects the data from individuals and then publishes valuable information for public use or specialized \textit{analysts}. It may publish aggregated information, statistics, or some analysis using data mining algorithms. That is very useful to provide better services, more effective marketing, or a population statistics publication.

However, most datasets contain private or sensitive information from individuals. Recent regulations on data privacy, such as \textit{General Data Protection Regulation (GPDR)} \cite{EUdataregulations2018} and \textit{Lei Geral de Proteção de Dados Pessoais (LGPD)} \cite{lgpd}, pose the requirement of anonymity. Specifically, they require that an individual's information be rendered anonymous so that the individual is no longer identifiable from the published information. In the literature, this process is known as \textit{data re-identification}.

Many examples show that naive anonymization, i.e., removing all explicit identifiers, does not prevent the re-identification of an individual from its data. \cite{narayanan2008robust,narayanan2009anonymizing}. To overcome that problem, many privacy models were designed with stricter privacy requirements. 

% The privacy model is placed between individuals and public users.

% One notable demonstration of re-identification was carried out by Narayanan et al . In this work, the authors proposed a de-anonymization technique and provided a practical analysis of the Netflix Prize dataset. With little auxiliary information, the privacy of the Netflix users was broken. Given $8$ movie ratings of a user where 2 of them can be completely wrong, and dates can have a 14-day error, $99\%$ of the records can be uniquely identified. 

% The fragility of naive anonymization was also shown in a case study involving crawled data from Flickr and Twitter in 2007/2008 \cite{narayanan2009anonymizing}. One-third of Flickr and Twitter's verifiable members could be recognized in the anonymous Twitter network with a $12\%$ error rate. 

One of the most well-known privacy models is \textit{k-anonymity} \cite{samarati1998generalizing,sweeney2002k}. It requires that a published information from individual should not be distinguishable from at least $k-1$ individuals in the release. Based on k-anonymity, other privacy models have been proposed as \textit{l-diversity} \cite{machanavajjhala2007diversity}, \textit{t-closeness} \cite{li2007t,li2009closeness} and \textit{$\delta$-presence} \cite{nergiz2007hiding}.

Those models have a common problem: they assume that the attacker has limited background knowledge. The attacker can acquire background information on many parts of the process: the algorithm used for anonymization, domain knowledge, or public records.

An example is a class of attack based on the principle of minimality which many algorithms satisfying k-anonymity had their privacy hurt \cite{cormode2010minimizing,jin2010algorithm,xiao2010transparent}. Then, other attacks have been developed for those traditional privacy models as the \textit{composition attack} \cite{ganta2008composition} and foreground knowledge attack \cite{wong2011can}.

\subsection{Differential Privacy}

\textit{Differential privacy} \cite{dwork2011differential,dwork2006calibrating} is the state-of-the-art formal definition for data release under strong privacy guarantees. It imposes near-indistinguishability on the released information whether an individual belongs to a sensitive database or not. It assumes that the attacker knows about $n-1$ records of the sensitive dataset except for the record that he/she is trying to learn about.

The fundamental intuition is that an analyst's query is answered by a \textit{randomized algorithm} that queries the private database and returns a randomized answer sampled from \textit{output distribution}. A randomized algorithm is a differentially private mechanism (also referred to as a mechanism in this work) if the probability distribution of the outputs does not change significantly based on the presence or absence of an individual. It ensures statistical guarantees against the inference of private information through the use of auxiliary information.

% \begin{figure}[!ht]    

%     \begin{tikzpicture}            
%         \node at (2.8,1) {$x$};
%         \node at (2.8,2) {$x'$};

%         \draw [->, ultra thick] (3.2,2) -- (5.4,1.7);
%         \draw [->, ultra thick] (3.2,1) -- (5.4,1.3);

%         \node at (7,-0.7) {$Pr[M(x)=r] \approx Pr[M(x')=r]$};

%         \draw (5.5,0) rectangle (9,3);
%         \node[align=center] at (7.2, 1.5) {Differentially \\ private \\ mechanism $M$};

%         \draw [->, ultra thick] (9.1,1.5) -- (10.5,1.5);
%         \node at (10.8,1.5) {$r$};
    
%     \end{tikzpicture}
	
%     \caption{Differentially private mechanism. A differentially private mechanism $M$ should produce any output $r$ with almost the same probability whether any single user is in the database ($x$) or not ($x'$).}    
% \end{figure}

All mechanisms strive to shape the output distribution such that the true answer and answers with high utility have a high probability of being sampled. Mechanisms that achieve that provide useful information to the analyst. The formal notion of utility is discussed later in this section.

Algorithms can achieve differential privacy by employing output perturbation, which releases the true output of a given non-private query $f$ with noise injected. The magnitude of the noise should be large enough to cover the identity of the individuals in the input database $x$. 

% For a numeric query (i.e., query with numeric output) $f$, the \textit{Laplace mechanism} \cite{dwork2006calibrating} is a well-known output perturbing private method. It adds numeric noise to the output of $f$ and calibrates the noise based only on $f$ and not on $x$. The amount of noise injected is proportional to the concept of \textit{global sensitivity}. The global sensitivity measures the worst case impact on $f$'s output of the addition or removal of an individual over the set of possible input databases. This may result in an unreasonably high amount of noise when $x$ is far from the database with the worst case impact, which is the case for many realistic databases. 

% Given that, our goal is to produce private algorithms that have low sensitivity to inject less noise and consequently having a better accuracy. So Nissim et al. \cite{nissim2007smooth} proposed the Smooth Sensitivity framework that adds instance-based noise calibrated as a function of $x$. They introduced the notion of \textit{local sensitivity}, which quantifies the impact of addition or removal of an individual for the database instance $x$, resulting in a lower bound to the global sensitivity. Many works use this notion to shrink the amount of noise added to release more useful statistical information \cite{blocki2013differentially,karwa2011private, kasiviswanathan2013analyzing,lu2014exponential, zhang2015private}.    

In this work, we focus on non-numeric queries, i.e., queries where the range is non-numeric. For instance, a query that returns the most frequent name from a database of people's names is non-numeric. In contrast, numeric queries return numeric answers, e.g., a query that returns the mean salary of the company's employees.

Given a non-numeric query $f: \domain \rightarrow \range$, where $\mathcal{R}$ is its non-numeric range, the \textit{exponential mechanism} \cite{mcsherry2007mechanism} achieves differential privacy by sampling elements from $\mathcal{R}$ based on the exponential distribution. This requires an \textit{utility function} $u(x,r)$ that takes as input a database $x$ and an element $r \in \mathcal{R}$ and outputs a numeric \textit{utility score} that measures the utility of $r$. The larger $u(x,r)$, the higher the probability of the exponential mechanism outputting $r$. For instance, in the \textit{most commom name} query, a reasonable utility function $u(x,r)$ returns the frequency of the name $r$ in the database $x$ as the utility score for $r$.

The noise added by the exponential mechanism is not numeric, so it is sampling noise. The exponential mechanism can sample a name that is not the most frequent, i.e., a name that does not have the best utility score. The amount of noise injected is proportional to the concept of \textit{global sensitivity}. The global sensitivity measures the worst-case impact on the utility function $u(x,r)$ of the addition or removal of an individual from $x$, for all databases $x$ and all $r \in \mathcal{R}$. Note that the global sensitivity does not depend on the input database. Given that, our goal is to produce private algorithms with low sensitivity to inject less noise and, consequently, have better accuracy. 

Example \ref{example:ebc} introduces the running example of this paper which is an application that selects influential node based on centrality metric on a graph. Centrality metrics measure a node's ability to communicate and spread information in the network. In this work, we use the Egocentric Betweenness Centrality (EBC) metric that indicates the power of intermediation of a node. Example \ref{example:example1} describes the global sensitivity concept in our running example.

\begin{example} (Running Example)
    Here we introduce the running example of this paper. Consider an application where, given a graph $G=(V,E)$, the analyst's non-numeric query should report the node with the largest EBC \cite{freeman1978centrality,marsden2002egocentric,everett2005ego}. The EBC metric measures the degree to which nodes stand between each other, defined as 

    $$ EBC(c) = \sum_{u,v \in N_c | u \neq v}  \frac{p_{uv}(c)}{q_{uv}(c)},$$

    where $N_c = \{ v \in V | \{c,v\} \in E \}$ is the set of neighbors of a given node $c$, $q_{uv}(c)$ is the number of shortest paths connecting $u$ and $v$ on the induced subgraph $G[N_c \cup \{ c\}]$ and $p_{uv}(c)$ is the number of those paths that include $c$.
    
    For instance, let $G$ be the graph illustrated in Figure \ref{fig:worst_graph}. Node $a$ has EBC score equal to $7.5$ since there are ${{6}\choose{2}}=15$ pairs of neighbors of the form $\{v_i,v_j\}$, for $0 \leq i < j \leq 5$, that each contributes with $0.5$ as they have two geodesic paths of length $2$ from $v_i$ to $v_j$, where only one contains $a$. Pairs of the form $\{ b,v_i \}$, for $0 \leq i \leq 5$ do not contribute to the score of $a$ since there is only one geodesic path (length $1$) from $b$ to $v_i$ and it does not contain $a$. 


    \begin{figure}[ht]    
        \centering
                
        \begin{tikzpicture}[]
            \foreach \pos/\name in {{(1.11,0)/a}, {(2.22,0)/b}, {(3.33,-1.5)/v_5}, {(2.67,-1.5)/v_4}, {(2,-1.5)/v_3}, {(1.34,-1.5)/v_2}, {(0.67,-1.5)/v_1}, {(0,-1.5)/v_0}}
            \node[vertex] (\name) at \pos {$\name$};
            
            \foreach \source/ \dest in {a/v_0, a/v_1, a/v_2, a/v_3, a/v_4, a/v_5, b/v_0, b/v_1, b/v_2, b/v_3, b/v_4, b/v_5}
            \path[edge] (\source) -- (\dest);    
            
            \path[dashed edge] (a) -- (b);
            
        \end{tikzpicture}        
    
        \caption{Egocentric betweenness sensitivity.}
        \label{fig:worst_graph}   
    \end{figure}
\label{example:ebc}
\end{example}


\begin{example} (Global Sensitivity)
    To compute global sensitivity, one should calculate the difference of utility scores $|u(x,r)-u(x',r)|$ for all pairs of databases $x$ and $x'$ that differ in one individual and for elements $r$ in the range of the numeric query. In our running example, the utility function is EBC and $x$ and $x'$ are graph databases. We use edge differential privacy where the information to be protect is the edges. Thus when computing $|u(x,r)-u(x',r)|$ for $x$ and $x'$ that differ in one edge.

    The global sensitivity is usually given in closed form formula. We show the complete development and proofs for that on Chapter \ref{chapter:node_influential_analysis}. However, to illustrate this example we show the pair $x$ and $x'$ that maximizes $|u(x,r)-u(x',r)|$. Let $x$ be the graph in Figure \ref{fig:worst_graph} and $x'$ be the graph obtained from $x$ by removing the edge $(a,b)$. The new EBC score of $a$ is $15$, $1$ point for each one of the $15$ pairs $\{ v_i, v_j \}$, $0 \leq i \leq 5$, as now there is only one geodesic path from $v_i$ to $v_j$ which includes $a$ (path $<v_i, a ,v_j>$). The paths of the form $<v_i, b, v_j>$ are not counted since $b$ no longer belongs to $N_a$. Thus, the global sensitivity is equal to $7.5$.
\label{example:example1}
\end{example}

In this application (Example \ref{example:example1}), the global sensitivity has a significant concern: the gadget found this example, formed by two nodes with a high degree that share all neighbors, and those neighbors do not have an edge to each other, is unlikely to be found in real-world graphs. Therefore, real-world graphs are far from the worst-case scenario, and mechanisms calibrated by the global sensitivity may be unreasonably large, which implies adding overwhelming amounts of noise.

For numeric queries, Nissim et al \cite{nissim2007smooth} proposed the smooth sensitivity framework that adds instance-based noise calibrated as a function of $x$. They introduced the notion of \textit{local sensitivity}, which quantifies the impact of addition or removal of an individual for the input database instance $x$, resulting in a lower bound to the global sensitivity. Note that the main difference between the global sensitivity and local sensitivity is that the first is not dependent on the input database $x$ and the latter is. Many works use this notion to reduce the amount of noise added to release more useful statistical information \cite{blocki2013differentially,karwa2011private,kasiviswanathan2013analyzing,lu2014exponential,zhang2015private}.

Example \ref{example:example1} shows how local sensitivity would be measured in the non-numeric graph application and that it is significantly smaller for more usual graphs.

% Local sensitivity may yield a lower value than the global sensitivity for many applications since it measures the impact of the addition or removal of an individual in 

% Example \ref{example:example1} shows local measurements

% For a numeric query (i.e., query with numeric output) $f$, the \textit{Laplace mechanism} \cite{dwork2006calibrating} is a well-known output perturbing private method. It adds numeric noise to the output of $f$ and calibrates the noise based only on $f$ and not on $x$. The amount of noise injected is proportional to the concept of \textit{global sensitivity}. The global sensitivity measures the worst case impact on $f$'s output of the addition or removal of an individual over the set of possible input databases. This may result in an unreasonably high amount of noise when $x$ is far from the database with the worst case impact, which is the case for many realistic databases. 

% So Nissim et al. \cite{nissim2007smooth} proposed the Smooth Sensitivity framework that adds instance-based noise calibrated as a function of $x$. They introduced the notion of \textit{local sensitivity}, which quantifies the impact of addition or removal of an individual for the database instance $x$, resulting in a lower bound to the global sensitivity. Many works use this notion to shrink the amount of noise added to release more useful statistical information \cite{blocki2013differentially,karwa2011private, kasiviswanathan2013analyzing,lu2014exponential, zhang2015private}.    



\begin{example} (Local Sensitivity Example)     
    In this instance (Figure \ref{fig:usual_ebc}), verify that the node $a$ has EBC score equal to $6.5$: 1 for each pair $\{v_0, v_2\}$, $\{v_0, v_3\}$, $\{v_0, b\}$, $\{v_1, v_2\}$, $\{v_1, v_3\}$ and $\{v_1, b\}$ and 0.5 for $\{v_2, v_3\}$. 
    
    The worst measurement of the sensitivity (difference of EBC when adding/removing an edge) the utility function for a node is given by removing the edge $(a,v_0)$. That reduces the EBC score of $a$ by only $3$ ($1$ for each pair $\{v_0, b\}$, $\{v_0, v_2\}$ and $\{v_0, v_3\}$ since $v_0$ is no longer a neighbor of $a$). This means that local sensitivity for this instance is 3, which is smaller than its global sensitivity.

    \begin{figure}[ht]
        \caption{Egocentric betweenness sensitivity - Local Sensitivity}
                    
        \centering
        
        \begin{tikzpicture}[]
            \foreach \pos/\name in {{(1.11,0)/a}, {(2.22,0)/b}, {(3.33,-1.5)/v_5}, {(2.67,-1.5)/v_4}, {(2,-1.5)/v_3}, {(1.34,-1.5)/v_2}, {(0.67,-1.5)/v_1}, {(0,-1.5)/v_0}}
            \node[vertex] (\name) at \pos {$\name$};
            
            \foreach \source/ \dest in {a/b, a/v_1, a/v_2, a/v_3, b/v_2, b/v_3, b/v_4, b/v_5, v_0/v_1, v_4/v_5}
            \path[edge] (\source) -- (\dest);    
            
            \path[dashed edge] (a) -- (v_0);
        \end{tikzpicture}
            
        \label{fig:usual_ebc}    
    \end{figure}
        

    % Consider the graph in Figure \ref{fig:grapha}. The removal of edge $(a,b)$ sets the traditional local sensitivity to $7.5$ which is also the case for global sensitivity. But measurements of sensitivity per node (element) are much smaller. For instance, the sensitivity for a node $v_i$ ($0 \leq i \leq 5$) is $1$ which is set by the removal of edge $(a,b)$ where $EBC(v_i)$ increases from $0$ to $1$ (path $<a,v_i,b>$). We explore this to improve the accuracy further.
    \label{example:example1}
\end{example} 

Furthermore, we identified that we could explore a more specific notion of local sensitivity which we call \textit{element local sensitivity}. Traditional local sensitivity measures the largest impact of the addition or deletion of an individual to the input database over all outputs $r \in \mathcal{R}$. Element local sensitivity computes this impact, but only for some given element $r \in \mathcal{R}$. That allows us to explore local measurements of the sensitivity of $f$ even if traditional local sensitivity is near the global sensitivity, but, for most elements in $\mathcal{R}$, the element local sensitivity is low. Example \ref{example:ebc_element_local} shows a case where element local sensitivity is significantly smaller than global and traditional local sensitivity for some elements $r \in \mathcal{R}$.

\begin{example} (Element Local Sensitivity)         
    Consider the graph in Figure \ref{fig:worst_graph}. The removal of edge $(a,b)$ sets the traditional local sensitivity to $7.5$ which is also the case for global sensitivity. But measurements of sensitivity per node (element) are much smaller. For instance, the sensitivity for a node $v_i$ ($0 \leq i \leq 5$) is $1$ which is set by the removal of edge $(a,b)$ where $EBC(v_i)$ increases from $0$ to $1$ (path $<a,v_i,b>$). 

    \label{example:ebc_element_local}
\end{example} 

A non-numeric mechanism applying local sensitivity could add less noise to the output than a global sensitivity-based approach. To the best of our knowledge, the literature lacks generic mechanisms that apply local sensitivity to non-numeric settings, which arises as a great research opportunity. 

This work introduces the local dampening mechanism, a novel framework to provide differential privacy for non-numeric queries using local sensitivity. Also, we extend the local dampening mechanism to provide better accuracy for element local sensitivity. We develop a theoretical accuracy analysis and a guide to construct accurate local dampening instances.


% The problem statement of this thesis is described in Section \ref{sec:problem_statement}. In Section \ref{sec:introduction_applications}, we introduce the two applications to the Local Dampening that we address in the work. The contributions are stated in Section \ref{sec:contributions}.
% In this thesis, we address the problem of releasing the output of a non-numeric function using differential privacy as stated in next section. For that we propose the Local Dampening mechanism, an output perturbing non-numeric differentially private mechanism that applies the notion of local sensitivity to shrink the amount of noise injected compared to traditional global sensitivity based approaches.


\section{Problem Statement}
\label{sec:problem_statement}

In this work, we address the problem of releasing the output of a non-numeric function using differential privacy. Let $x$ be a sensitive database and $f$ a non-numeric function to be evaluated on $x$. The database is represented as vector $x \in \mathcal{D}^n$ where each entry represents an individual tuple, and $\mathcal{D}$ is the set of all possible tuple values. The function $f: \mathcal{D}^n \rightarrow \mathcal{R}$ receives the dataset $x \in \mathcal{D}^n$ to be evaluated and outputs an element $r$ in its non-numeric range $\mathcal{R}$.

The task is to release the output $f(x)$ without leaking much information about the individuals using differential privacy. For that, we need to design a randomized algorithm $\mathcal(A)(x)$ that adds noise to $f(x)$ such that it satisfies the formal definition of differential privacy (Definition \ref{def:dp}).

The exponential mechanism is an example of a mechanism that uses this setup. A mechanism that addresses this problem is a natural building block to compose other complex private algorithms and can potentially be used in any work in the literature that uses the exponential mechanism as in \cite{zhang2017privbayes,friedman2010data,mcsherry2009privacy,mohammed2011differentially,hardt2012simple}. 


\section{Applications}
\label{sec:introduction_applications}


We illustrate the effectiveness of our approach by applying it to three very different problems: median selection, influential node analysis, and decision tree induction.

\textbf{Median selection.} Median selection is a commonly addressed problem to show the accuracy of differentially private mechanisms. The task is to report the label of the median element in a given database.

\textbf{Influential node analysis.} Identifying influential nodes in a network is an important task for social network marketing \cite{ma2008mining}. The goal is to search for central nodes in a graph database. Given a centrality/influence metric, we release the label of the top-k most central nodes while preserving the privacy of the relationships between nodes in the graph. In this work, we use EBC as an influence metric. EBC metric identifies influential nodes that are important in different loosely connected parties. This is the graph application shown in Examples \ref{example:example1}, \ref{example:example1} and \ref{example:ebc_element_local}.

\textbf{Decision tree induction}. We tackle a data mining problem which is constructing decision trees for classification. We provide a private adaptation to the ID3 algorithm to build a decision tree from a given tabular dataset. For the automatic tree induction, we use IG as the split criterion for choosing an attribute to branch.

% Many purity measures are used to decide how to split the nodes in the decision tree. In this work, we use \gls{IG} and \gls{Gini} as split criterion.


\section{Thesis Contribution}
\label{sec:contributions}


Most of the contributions of this paper were previously published in our paper \cite{DBLP:journals/pvldb/FariasBFMMS20}:

\begin{itemize}
    \item FARIAS, V. A. E. de; BRITO, F. T.; FLYNN, C.; MACHADO, J. C.; MAJUMDAR, S.;SRIVASTAVA, D. Local dampening:  Differential privacy for non-numeric queries via local sensitivity. Proc. VLDB Endow., v. 14, n. 4, p. 521–533, 2020. Available in: http://www.vldb.org/pvldb/vol14/p521-farias.pdf.
\end{itemize}

The main contributions of this paper are the following:

\begin{itemize}
    \item We adapt the concept of local sensitivity originally defined for the numeric setting to the non-numeric setting.
    \item We introduce the notion of element local sensitivity to the non-numeric setting, which is a specialized definition of local sensitivity where the sensitivity is measured for a single element in the range of the function to be evaluated.
    \item We propose the \textit{local dampening mechanism}, an output perturbing non-numeric differentially private mechanism that applies the notion of local sensitivity for the non-numeric setting to attenuate the utility function in order to reduce the amount of noise injected compared to traditional global sensitivity based approaches. Local dampening also employs the exponential distribution as the exponential mechanism. 
    \item We present the second version of our approach named the shifted local dampening mechanism, which can effectively use the element local sensitivity to improve accuracy.
    \item We develop a theoretical and empirical accuracy analysis where we enumerate some conditions in which the local dampening mechanism benefits from the local sensitivity notions. Under those conditions, we show that the exponential mechanism is an instance of the local dampening mechanism, and it is the worst instance of the local dampening mechanism in terms of accuracy. Also, we discuss the scenario where those conditions are not met and how we can still have good accuracy.
    \item We tackle the median selection problem where a private mechanism should report the label of the median element. Empirical results show that the local dampening mechanism can improve up to $29\%$ about global sensitivity approaches.
    \item We apply the local dampening mechanism to construct differentially private algorithms for a graph problem called Influential Node Analysis using Egocentric Betweenness Centrality as the influence metric, and we show how to compute local sensitivity for this application. Experimental results show that our approach could be as accurate as global sensitivity-based mechanisms using $2$ to $4$ orders of magnitude less privacy budget than global sensitivity-based approaches. 
    \item We address the application of building private algorithms for decision tree induction as an example data-mining application for tabular data. We present a differentially private adaptation of the entropy-based ID3 algorithm using the local dampening mechanism, and we provide a way to compute the local sensitivity efficiently. We can improve accuracy up to $5\%$ compared to previous works.
\end{itemize}


\section{Thesis Organization}


The remainder of this thesis is organized as follows. In Chapter \ref{chapter:preliminaries}, we introduce the main concepts of differential privacy. Particularly, we present the definition of differential privacy, non-numeric differential privacy, the notions of global and local sensitivity, and the composition theorems.

Chapter \ref{chapter:local_dampening} describes the essential elements that compose this thesis: the element local sensitivity, admissible functions, and the dampening function of the utility function. Given that, we propose the local dampening mechanism and prove it to be differentially private. Also, we present the related work, the well-known exponential mechanism, and permute-and-flip.

In Chapter \ref{chapter:shifted_local_dampening}, we introduce the shifted local dampening mechanism. We analyze some problems of the original local dampening mechanism and how the shifted local dampening aims to solve them. Also, we provide an accuracy analysis where we show theoretical analysis and a guide to build a good shifted local dampening instance.

The median selection problem is tackled in Chapter \ref{chapter:median_selection}. In Chapter \ref{chapter:node_influential_analysis}, we apply the local dampening mechanism to the influential node analysis problem using EBC and present the related work to this application. Chapter \ref{chapter:decision_tree_induction} address the decision tree induction problem using IG as the split criterion and also present the related work for this problem.

Finally, Chapter \ref{chapter:conclusion} we draw conclusions and propose future works based on this work.
